Tight Regret Bounds for Infinite-armed Linear Contextual Bandits

Linear contextual bandit is an important class of sequential decision making problems with a wide range of applications to recommender systems, online advertising, healthcare, and many other machine learning related tasks. While there is a lot of prior research, tight regret bounds of linear contextual bandit with infinite action sets remain open. In this paper, we address this open problem by considering the linear contextual bandit with (changing) infinite action sets. We prove a regret upper bound on the order of $O(\sqrt{d^2T\log T})\times \text{poly}(\log\log T)$ where $d$ is the domain dimension and $T$ is the time horizon. Our upper bound matches the previous lower bound of $\Omega(\sqrt{d^2 T\log T})$ in [Li et al., 2019] up to iterated logarithmic terms.

==> single-step-regret.tex <==
\subsection{Regret upper bound at a single time step}

For each time $t$, we first bound the expected error of the estimation of any arm that lies out of its confidence band.

% The key to proving Lemma~\ref{lem:single-step-regret} is the following reward error bound for the selected arm at time $t$, which is also in an expectation form.

\begin{lemma}\label{lem:reward-error-bound-in-each-layer}
There exists a sufficiently large universal constant $C > 0$ such that for each layer $\zeta \in \{0, 1, 2, \dots, \zeta_0\}$, 
for each time $t \in [T]$, and for any $\delta \in (0, 1/2]$,  it holds that
\begin{align}\label{eq:reward-error-bound-in-each-layer}
\E\left[\max_{x \in D_t} \left\{\mathbf{1}\left[ \left| x^\top (\hat{\theta}_{\zeta, t} - \theta)\right| 
\geq  C \sqrt{d } \cdot  \alpha_{\zeta, t}^{x}  \cdot \omega_{\zeta, t}^{x}  \right]
\cdot \left| x^\top (\hat{\theta}_{\zeta, t} - \theta)\right| \right\} \right] 
\lesssim \delta d / \sqrt{T \ln^2 T}.
\end{align}
\end{lemma}


To prove Lemma~\ref{lem:reward-error-bound-in-each-layer}, we adopt a novel argument that partitions the action set according to the geometric scale of the confidence levels of the actions. Using Corollary~\ref{cor:uniform-tail-bound}, for each partition, we derive a uniform error bound that for the actions in the partition. Since we have no control on the index of the partition that the maximizer $x^*$ belongs to, we finally employ a union bound argument to combine the error bounds for every partition and complete the proof. 

% It is worthwhile to note that a similar partitioning approach has been used in the algorithms for linear contextual bandits with finite-sized action sets (e.g., \cite{auer2002using,chu2011contextual,li2019near}). However, previous algorithms explicitly partition the action set, while in our work, the partitioning idea only appears in the proof. Furthermore, our proof technique is very different from the previous works.

\begin{proof}[Proof of Lemma~\ref{lem:reward-error-bound-in-each-layer}]
For each layer $\zeta$ 
and for each time $t$,
consider a partition of $D_t$, namely 
$\{\calA_{\zeta, t}^{\kappa}\}_{\kappa \in \{1, 2, 3, \dots, K\}}$, 
where $K = \lceil \log_2 (T^2 /\delta^2)\rceil + 1$, and we define
\begin{align*}
\calA_{\zeta, t}^{\kappa} =  \left\{
\begin{array}{ll}
\{x\in D_t : \omega_{\zeta, t}^x \in (2^{-\kappa}, 2^{-\kappa + 1}]\} & \text{when~} \kappa \in \{1, 2, 3, \dots, K - 1\}\\
\{x\in D_t : \omega_{\zeta, t}^x \in (0, 2^{-\kappa + 1}]\}  & \text{when~} \kappa = K
 \end{array}
\right. .
\end{align*}
For each $\kappa$, we let 
\[
m_{\zeta, t}^\kappa = \sup_{i \in \calA_{\zeta, t}^{\kappa}} \left\{\left| x_{it}^\top (\hat{\theta}_{\zeta,t} - \theta)\right|\right\}
\]
be the maximum estimation error for the context vectors in $\calA_{\zeta, t}^{\kappa}$. 
By Corollary~\ref{cor:uniform-tail-bound}, there exists a universal constant $C$, 
such that for all $\beta \geq \sqrt{\ln 2}$, we have that 
\begin{align*}
\Pr\left[ m_{\zeta, t}^\kappa \geq C \cdot 2^{-\kappa} \sqrt{d} \cdot \beta\right] &= \Pr\left[ m_{\zeta, t}^\kappa \geq (C/2) \cdot 2^{-\kappa + 1} \sqrt{d} \cdot \beta\right] \\
& \leq \Pr\left[ \exists i \in \calA_{\zeta, t}^{\kappa}:   \left| x_{it}^\top (\hat{\theta}_{\zeta, t} - \theta)\right| 
\geq (C/2) \cdot  \omega_{\zeta, t}^i \sqrt{d} \cdot \beta\right] \leq e^{-\beta^2} .
\end{align*}

\iffalse
Now we let $\alpha_t^\kappa = \sqrt{\max\{1, {\ln [T \ln^4 T \cdot 2^{-2\kappa}/d]}\}}$, and use $\mathbf{1}[\cdot] $ to denote the indicator function. For each $\kappa$, it holds that
\begin{align}
&\E \left[ \mathbf{1} \left[ m_{\zeta, t}^\kappa \geq C \cdot 2^{-\kappa} 
\sqrt{d } \cdot \left( \alpha_t^{\kappa} + \sqrt{\ln (1/\delta)}\right) \right] \cdot m_{\zeta, t}^\kappa \right] \nonumber \\
\leq\ & \Pr\left[m_{\zeta, t}^\kappa \geq C \cdot 2^{-\kappa} \sqrt{d } \cdot  \left( \alpha_t^{\kappa} + \sqrt{\ln (1/\delta)}\right)  \right] 
\cdot \left( C \cdot 2^{-\kappa} \sqrt{d } \cdot  \left( \alpha_t^{\kappa} + \sqrt{\ln (1/\delta)}\right)  \right)  \nonumber\\
& \qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad + \int_{C \cdot 2^{-\kappa} \sqrt{d } \cdot \alpha_t^{\kappa} }^{+\infty} \Pr[m_{\zeta, t}^\kappa \geq z] dz  \nonumber \\
\leq\ &  \exp\left(- (\alpha_t^\kappa + \sqrt{\ln (1/\delta)})^2\right)  \cdot C \cdot 2^{-\kappa} \sqrt{d} \cdot  \left( \alpha_t^{\kappa} + \sqrt{\ln (1/\delta)}\right)  
+ C \cdot 2^{-\kappa} \sqrt{d} \cdot 
\int_{\alpha_t^\kappa + \sqrt{\ln (1/\delta)}}^{\infty} e^{-\beta^2} d\beta  \nonumber \\
\lesssim\ & \exp\left(- (\alpha_t^\kappa+\sqrt{\ln (1/\delta)})^2\right)  \cdot 2^{-\kappa} \sqrt{d} \cdot \left(\alpha_t^{\kappa} + \sqrt{\ln (1/\delta)}\right) \nonumber \\
\leq\ &\delta  \exp\left(- (\alpha_t^\kappa)^2\right) \cdot 2^{-\kappa} \sqrt{d} \cdot \left(\alpha_t^{\kappa} + \sqrt{\ln (1/\delta)}\right) . \label{eq:lem-reward-error-bound-1}
\end{align}

\fi




Now we let $\alpha_t^\kappa = \sqrt{\max\{1, {\ln [T \ln^4 T \ln^2(1/\delta) \cdot 2^{-2\kappa}/(d\delta^2)]}\}}$, and use $\mathbf{1}[\cdot] $ to denote the indicator function. For each $\kappa$, it holds that
\begin{align}
&\E \left[ \mathbf{1} \left[ m_{\zeta, t}^\kappa \geq C \cdot 2^{-\kappa} 
\sqrt{d} \cdot \alpha_t^{\kappa} \right] \cdot m_{\zeta, t}^\kappa \right] \nonumber \\
\leq\ & \Pr\left[m_{\zeta, t}^\kappa \geq C \cdot 2^{-\kappa} \sqrt{d} \cdot \alpha_t^{\kappa} \right] 
\cdot \left( C \cdot 2^{-\kappa} \sqrt{d} \cdot \alpha_t^{\kappa} \right) 
+ \int_{C \cdot 2^{-\kappa} \sqrt{d} \cdot \alpha_t^{\kappa} }^{+\infty} \Pr[m_{\zeta, t}^\kappa \geq z] dz  \nonumber \\
\leq\ &  \exp\left(- (\alpha_t^\kappa)^2\right)  \cdot C \cdot 2^{-\kappa} \sqrt{d} \cdot \alpha_t^{\kappa} 
+ C \cdot 2^{-\kappa} \sqrt{d} \cdot 
\int_{\alpha_t^\kappa}^{\infty} e^{-\beta^2} d\beta  \nonumber \\
\lesssim\ & \exp\left(- (\alpha_t^\kappa)^2\right)  \cdot 2^{-\kappa} \sqrt{d} \cdot \alpha_t^{\kappa}. \label{eq:lem-reward-error-bound-1}
\end{align}

We now upper bound Eq.~\eqref{eq:lem-reward-error-bound-1} by considering the following two cases.
In the first case, when $\alpha_t^\kappa = 1$, 
we have that $T \ln^4 T \ln^2(1/\delta) \cdot 2^{-2\kappa}/(d\delta^2) \leq e$, 
i.e., $2^{-\kappa} \lesssim \sqrt{d \delta^2 / (T \ln^4 T \ln^2(1/\delta))}$. 
Therefore, Eq.~\eqref{eq:lem-reward-error-bound-1} is upper bounded by $e^{-1} \cdot 2^{-\kappa} \sqrt{d}  \lesssim \delta d  /\sqrt{T\ln^4 T \ln^2(1/\delta)}$. 
In the second case, when $\alpha > 1$, we have that 
$T \ln^4 T \ln^2(1/\delta) \cdot 2^{-2\kappa}/(d\delta^2) = \exp((\alpha_{t}^{\kappa})^2)$ 
and therefore 
$2^{-\kappa} = \delta \sqrt{d/(T\ln^4 T \ln^2(1/\delta))} \cdot \exp((\alpha_{t}^{\kappa})^2/2)$. 
We can upper bound Eq.~\eqref{eq:lem-reward-error-bound-1} by 
$\exp\left(-(\alpha_t^\kappa)^2 (1 - 1/2)\right) \cdot \delta \sqrt{d/(T\ln^4 T \ln^2(1/\delta))}
\cdot  \sqrt{d} \cdot \alpha_t^{\kappa}  \lesssim \delta d/\sqrt{T\ln^4 T \ln^2(1/\delta)}$. 
Summarizing the two cases, we have 
\begin{align}
&\E \left[ \mathbf{1} \left[ m_{\zeta, t}^\kappa 
\geq C \cdot 2^{-\kappa} \sqrt{d} \cdot \alpha_t^{\kappa} \right] 
\cdot m_{\zeta, t}^\kappa \right] 
\lesssim \delta d /\sqrt{T \ln^4 T \ln^2(1/\delta)} . \label{eq:lem-reward-error-bound-2}
\end{align}

We now work with the Left-Hand Side of Eq.~\eqref{eq:reward-error-bound-in-each-layer}. Let $x^*$ be the maximizer in the LHS of Eq.~\eqref{eq:reward-error-bound-in-each-layer}, and let $\kappa^*$ be the index of the partition such that $x^* \in \calA_{\zeta, t}^{\kappa^*}$. We have 
\begin{align}
& \E\left[\mathbf{1}\left[ \left| (x^*)^\top (\hat{\theta}_{\zeta, t} - \theta)\right| \geq  C \sqrt{d} \cdot \alpha_{\zeta, t}^{x^*} \omega_{\zeta, t}^{x^*}  \right]
\left| (x^*)^\top (\hat{\theta}_{\zeta, t} - \theta)\right|\right] \nonumber\\
 \leq \ & \E\left[\mathbf{1}\left[\kappa^* = K\right] \cdot   \left| (x^*)^\top (\hat{\theta}_{\zeta, t} - \theta)\right| \right] \nonumber \\
&  \qquad  + \E\left[\mathbf{1}\left[\kappa^* < K\right] \cdot \mathbf{1}\left[ \left| (x^*)^\top (\hat{\theta}_{\zeta, t} - \theta)\right| 
\geq  C \sqrt{d} \cdot \alpha_{\zeta, t}^{x^*} \omega_{\zeta, t}^{x^*}  \right] \cdot \left| (x^*)^\top (\hat{\theta}_{\zeta, t} - \theta)\right|\right] . \label{eq:lem-reward-error-bound-3}
\end{align}


We first focus on the first term in the Right-Hand Side of Eq.~\eqref{eq:lem-reward-error-bound-3}.  When $\kappa^* = K$, we have $\omega_{\zeta, t}^{x^*} \leq 2/(T/\delta)^2$. Therefore, 
\begin{align*}
&\Pr\left[\kappa^* = K ~\text{and}~  \left| (x^*)^\top (\hat{\theta}_{\zeta, t} - \theta)\right| 
\geq  \delta/\sqrt{T  \ln^4 T \ln^2(1/\delta)} \right] \\
& \qquad\qquad \qquad \leq \Pr\left[   (\omega_{\zeta, t}^{i^*})^{-1} \left| (x^*)^\top (\hat{\theta}_{\zeta, t} - \theta)\right| >T^{1.5}/(2 \delta \ln^2 T \ln (1/\delta))   \right] \lesssim \delta^3 \cdot \exp(-T),
\end{align*}
where the last inequality is due to Corollary~\ref{cor:uniform-tail-bound} and for $T \gtrsim \sqrt{d}$. Therefore, we have
\begin{align}
 &\E\left[\mathbf{1}\left[\kappa^* = K\right] \left| (x^*)^\top (\hat{\theta}_{\zeta, t} - \theta)\right| \right]  \nonumber \\
 \lesssim \ & \delta /\sqrt{T \ln^4 T \ln^2(1/\delta)}  \nonumber \\
 & \qquad + \E\left[\mathbf{1}\left[\kappa^* = K ~\text{and}~ \left| (x^*)^\top (\hat{\theta}_{\zeta, t} - \theta)\right| > \delta/\sqrt{T \ln^4 T \ln^2(1/\delta)}\right]  \cdot  \left| (x^*)^\top (\hat{\theta}_{\zeta, t} - \theta)\right|  \right]  \nonumber\\
 \leq \ & \delta/ \sqrt{T \ln^4 T \ln^2(1/\delta)} \nonumber \\
 & \qquad +  \sqrt{\Pr\left[\kappa^* = K ~\text{and}~ \left| (x^*)^\top (\hat{\theta}_{\zeta, t} - \theta)\right| > \delta/\sqrt{T \ln^4 T \ln^2(1/\delta)}\right]  \cdot  \E\left[ \left| (x^*)^\top (\hat{\theta}_{\zeta, t} - \theta)\right|^2  \right] } \nonumber\\
 \lesssim \ & \delta / \sqrt{T \ln^4 T \ln^2(1/\delta)},  \label{eq:lem-reward-error-bound-6}
\end{align}
where the second inequality due to Cauchy-Schwartz, and the last inequality is because of 
\[
\E\left[ \left| (x^*)^\top (\hat{\theta}_{\zeta, t} - \theta)\right|^2\right] \leq \E\left[ \left\| \hat{\theta}_{\zeta, t} - \theta\right\|_2^2\right] \leq \E\left[\left( \left\| \hat{\theta}_{\zeta, t}\right\|_2 + 1\right)^2\right] \lesssim T^2 .
\]

Now we work with the second term in the Right-Hand Side of Eq.~\eqref{eq:lem-reward-error-bound-3}.  When $\kappa^* < K$, we have  $2^{-\kappa^*} < \omega_{\zeta, t}^{x^*}$ and $\alpha_t^{\kappa^*} \leq \alpha_{\zeta, t}^{x^*}$, and therefore 
\begin{align}
&\mathbf{1}\left[\kappa^* < K\right] \cdot \mathbf{1}\left[ \left| (x^*)^\top (\hat{\theta}_{\zeta, t} - \theta)\right| 
\geq  C \sqrt{d} \cdot \alpha_{\zeta, t}^{x^*} \cdot \omega_{\zeta, t}^{x^*}  \right] \cdot \left| (x^*)^\top (\hat{\theta}_{\zeta, t} - \theta)\right| \nonumber \\
\leq\ & \mathbf{1}\left[ \left| (x^*)^\top (\hat{\theta}_{\zeta, t} - \theta)\right| 
\geq C \sqrt{d} \cdot \alpha_{\zeta, t}^{x^*}\cdot 2^{-\kappa^*}  \right] 
\cdot \left| (x^*)^\top (\hat{\theta}_{\zeta, t} - \theta)\right| \nonumber \\
\leq\ &  \mathbf{1}\left[ m_{t}^{\kappa^*}
\geq C \sqrt{d} \cdot \alpha_{\zeta, t}^{x^*}
\cdot 2^{-\kappa^*}  \right] \cdot m_t^{\kappa^*} 
\leq \sum_{\kappa = 1}^{K-1} \mathbf{1}\left[ m_{t}^{\kappa}
\geq C \sqrt{d} \cdot \alpha_{\zeta, t}^{x^*} \cdot 2^{-\kappa^*}  \right] \cdot m_{\zeta, t}^\kappa . \label{eq:lem-reward-error-bound-4}
\end{align}
Taking expectation and invoking Eq.~\eqref{eq:lem-reward-error-bound-2}, we have 
\begin{align}
\E\left[\mathbf{1}\left[\kappa^* < K\right] \cdot 
\mathbf{1}\left[ \left| (x^*)^\top (\hat{\theta}_{\zeta, t} - \theta)\right| 
\geq  C \sqrt{d} \cdot \alpha_{\zeta, t}^{x^*} \cdot \omega_{\zeta, t}^{x^*}  \right] 
\cdot \left| (x^*)^\top (\hat{\theta}_{\zeta, t} - \theta)\right|\right] \nonumber\\
\leq \sum_{\kappa = 1}^{K - 1} 
\E\left[ \mathbf{1}\left[ m_{t}^{\kappa}
\geq C \sqrt{d} \cdot \alpha_{\zeta, t}^{x^*} \cdot 2^{-\kappa^*}  \right] \cdot m_{\zeta, t}^\kappa\right] 
\lesssim \delta d / \sqrt{T \ln^2 T} .
 \label{eq:lem-reward-error-bound-5}
\end{align}
Combining Eq.~\eqref{eq:lem-reward-error-bound-3}, Eq.~\eqref{eq:lem-reward-error-bound-6}, and Eq.~\eqref{eq:lem-reward-error-bound-5}, we have
\begin{align*}
\E\left[\mathbf{1}\left[ \left| (x^*)^\top (\hat{\theta}_{\zeta, t} - \theta)\right| 
\geq C \sqrt{d} \cdot \alpha_{\zeta, t}^{x^*} \cdot \omega_{\zeta, t}^{x^*} \right]
\cdot \left| (x^*)^\top (\hat{\theta}_{\zeta, t} - \theta)\right|\right] 
\lesssim \delta d / \sqrt{T \ln^2 T},
\end{align*}
proving the desired upper bound.
\end{proof}





For any layer $\zeta \in \{0, 1, 2, \dots, \zeta_0\}$ and any time period $t \in [T]$, we define 
\[
\overline m_{\zeta,t} := \max_{x\in\mathcal N_{\zeta,t}} \{ x^\top\theta \}, \qquad \text{and}\qquad
\underline m_{\zeta,t} := \min_{x\in\mathcal N_{\zeta,t}} \{ x^\top\theta \}
\]
as the largest and smallest mean reward for actions in the action subset $\mathcal N_{\zeta,t}$.
For convenience, we also define $\overline m_{\zeta_0+1,t} := \overline m_{\zeta_0,t}$ and $\underline m_{\zeta_0+1,t}:=\underline m_{\zeta_0,t}$.

Note that $\max_{x\in D_t} \{x^\top\theta \} = \overline m_{0,t}$ and $x_{t}^\top\theta \geq \underline m_{\zeta_t,t}$ (due to $x_t\in\mathcal N_{\zeta_t,t}$), we have that the regret incurred at time $t$ is
\begin{align}\label{eq:regret-time-t-mt}
\max_{x\in D_t}\{x^\top\theta\} - x_t^\top \theta \leq  \left((\overline m_{0,t}-\overline m_{\zeta_t,t}) + (\overline m_{\zeta_t,t}-\underline m_{\zeta_t,t})\right) \leq (\overline m_{\zeta_t,t}-\underline m_{\zeta_t,t}) + \sum_{\zeta = 1}^{\zeta_t} (\overline m_{\zeta-1,t}-\overline m_{\zeta,t}) .
\end{align}

In the following lemma, we provide upper bounds for the expressions in the Right-Hand Side of Eq.~(\ref{eq:regret-time-t-mt}).

\begin{lemma}\label{lem:mt}
For all $t$ and $\zeta=0,1,\cdots,\zeta_0$, it holds that
\begin{align}
& \mathbb E\left[\max\{\overline m_{\zeta,t}-\overline m_{\zeta+1,t} ,0\}\right] 
\lesssim \delta d / \sqrt{T \ln^2 T};\label{eq:mt-1}\\
& \mathbb E\left[ \max\{\overline m_{\zeta,t}-\underline m_{\zeta,t} - 2^{3-\zeta}, 0\}\right] 
\lesssim \delta  d / \sqrt{T \ln^2 T}.\label{eq:mt-2}
\end{align}
\end{lemma}

\begin{proof}
We first prove Eq.~(\ref{eq:mt-1}). Let $y^*_t := \arg\max_{y\in\mathcal N_{\zeta,t}}\{y^\top\theta\}$ and $z^*_t := \arg\max_{z\in\mathcal N_{\zeta,t}}\{z^\top\hat\theta_{\zeta,t} \}$.
If $y^*_t\in\mathcal N_{\zeta+1,t}$, then $\overline m_{\zeta,t}=\overline m_{\zeta+1,t}$ because $\mathcal N_{\zeta+1,t}\subseteq\mathcal N_{\zeta,t}$.
%Therefore, we only need to consider the case of $i^*_t\notin\mathcal N_{\zeta+1,t}$ for the sake of proving Eq.~(\ref{eq:mt-1}).
On the other hand, if $y^*_t\notin\mathcal N_{\zeta+1,t}$,
note that $z^*_t\in\mathcal N_{\zeta+1,t}$ because $z^*_t$ maximizes $z^\top\hat\theta_{\zeta,t}$
in $\mathcal N_{\zeta,t}$.
%, and for any $k\in\mathcal N_{\zeta,t}$ we have $\varpi_{\zeta,t}^k\leq 2^{-\zeta}$, 
%and hence $x_{j^*_t,t}^\top\hat\theta_{\zeta,t} \geq x_{kt}^\top\hat\theta_{\zeta,t} - \varpi_{\zeta,t}^{j^*_t} - \varpi_{\zeta,t}^k \geq x_{kt}^\top\hat\theta_{\zeta,t}-2^{1-\zeta}$ for all $k\in\mathcal N_{\zeta,t}$.
Summarizing both cases of $y^*_t\in\mathcal N_{\zeta+1,t}$ (in which $\overline m_{\zeta+1,t}=\overline m_{\zeta,t}$)
and $y^*_t\notin\mathcal N_{\zeta+1,t}$ (in which $\overline m_{\zeta+1,t}\geq (z^*_t)^\top\theta$ as $z^*_t\in\mathcal N_{\zeta+1,t}$), we have
\begin{equation}
\overline m_{\zeta,t} -\overline m_{\zeta+1, t} \leq \vct 1\{y^*_t\notin\mathcal N_{\zeta+1,t}\}\cdot (y^*_t-z^*_t)^\top\theta.
\label{eq:mm1-eq1}
\end{equation}

For any $\zeta,t$ and $y\in\mathcal N_{\zeta,t}$, define
$
\mathcal E_{\zeta,t}^y := \{|y^\top(\hat\theta_{\zeta,t}-\theta)| \leq \varpi_{\zeta,t}^y\}
$
as the success event in which the estimation error of $y^\top\hat\theta_{\zeta,t}$ for $y^\top\theta$ is within the confidence interval $\varpi_{\zeta,t}^y$.
By definition, 
\begin{align}
(y_t^*)^\top\theta &\leq (y_t^*)^\top\hat\theta_{\zeta,t} + \varpi_{\zeta,t}^{y^*_t} + \vct 1\{\neg\mathcal E_{\zeta,t}^{y^*_t}\}\cdot \big|(y_t^*)^\top(\hat\theta_{\zeta,t}-\theta)\big|;\label{eq:xistar-expansion}\\
(z_t^*)^\top\theta &\geq (z_t^*)^\top\hat\theta_{\zeta,t} - \varpi_{\zeta,t}^{z^*_t} - \vct 1\{\neg\mathcal E_{\zeta,t}^{z^*_t}\}\cdot \big|(z_t^*)^\top(\hat\theta_{\zeta,t}-\theta)\big|.
\label{eq:xjstar-expansion}
\end{align}
Also, conditioned on the event $y^*_t\notin\mathcal N_{\zeta+1,t}$, the procedure of Algorithm \ref{alg:suplinucb} implies 
\begin{equation}
(y_t^*)^\top\hat\theta_{\zeta,t} < (z_t^*)^\top\hat\theta_{\zeta,t} - 2^{1-\zeta}.
\label{eq:xijstar-side}
\end{equation}
Subtracting Eq.~(\ref{eq:xjstar-expansion}) from Eq.~(\ref{eq:xistar-expansion}) and considering Eq.~(\ref{eq:xijstar-side}), we have
\begin{align}
(y_t^*-z_t^*)^\top\theta
&\leq \varpi_{\zeta,t}^{y^*_t} + \varpi_{\zeta,t}^{z^*_t} - 2^{1-\zeta} + \sum_{x\in\{y^*_t,z^*_t\}}\vct 1\{\neg\mathcal E_{\zeta,t}^{x}\}\cdot \big|x^\top(\hat\theta_{\zeta,t}-\theta)\big|\nonumber\\
&\leq \sum_{x\in\{y^*_t,z^*_t\}}\vct 1\{\neg\mathcal E_{\zeta,t}^{x}\}\cdot \big|x^\top(\hat\theta_{\zeta,t}-\theta)\big|,
\label{eq:xijstar-main}
\end{align}
where the last inequality holds because $\varpi_{\zeta,t}^x\leq 2^{-\zeta}$ for all $x\in\mathcal N_{\zeta,t}$, if the algorithm is executed to level $\zeta+1$.
Combining Eqs.~(\ref{eq:mm1-eq1},\ref{eq:xijstar-main}) and Lemma \ref{lem:reward-error-bound-in-each-layer}, 
taking expectations, we obtain
\begin{align*}%\label{eq:mt1-eq2}
&\mathbb E\left[\max\{\overline m_{\zeta,t}-\overline m_{\zeta+1,t}, 0\}\right] \\
\leq\ & \mathbb E\left[\vct 1\{y^*_t\notin\mathcal N_{\zeta+1,t}\}\cdot \left(\vct 1\{\neg\mathcal E_{\zeta,t}^{y^*_t}\} \big|(y_t^*)^\top(\hat\theta_{\zeta,t}-\theta)\big|+\vct 1\{\neg\mathcal E_{\zeta,t}^{z^*_t}\} \big|(z_t^*)^\top(\hat\theta_{\zeta,t}-\theta)\big|\right)\right]\nonumber\\
\leq\ & \mathbb E\left[\vct 1\{\neg\mathcal E_{\zeta,t}^{y^*_t}\} \big|(y_t^*)^\top(\hat\theta_{\zeta,t}-\theta)\big|\right]+\mathbb E\left[\vct 1\{\neg\mathcal E_{\zeta,t}^{z^*_t}\} \big|(z_t^*)^\top(\hat\theta_{\zeta,t}-\theta)\big|\right] \nonumber
\lesssim \delta d / \sqrt{T \ln^2 T}.
\end{align*}

Now we focus on Eq.~(\ref{eq:mt-2}). We only need to prove the equation for $\zeta > 0$ since it is trivially true for $\zeta = 0$. Let $w^*_t := \arg\min_{w\in\mathcal N_{\zeta,t}}\{w^\top\theta\}$.
Clearly $\overline m_{\zeta,t}-\underline m_{\zeta,t}=(y_t^*-w_t^*)^\top\theta$.
Similar to Eqs.~(\ref{eq:xistar-expansion},\ref{eq:xjstar-expansion}), we can establish that
\begin{align}
(y_t^*)^\top\theta &\leq (y_t^*)^\top\hat\theta_{\zeta-1,t} + \varpi_{\zeta-1,t}^{y^*_t} + \vct 1\{\neg\mathcal E_{\zeta-1,t}^{y^*_t}\}\cdot \big|(y_t^*)^\top(\hat\theta_{\zeta-1,t}-\theta)\big|;\label{eq:xistar-expansion-2}\\
(w_t^*)^\top\theta &\geq (w_t^*)^\top\hat\theta_{\zeta-1,t} - \varpi_{\zeta-1,t}^{w^*_t} - \vct 1\{\neg\mathcal E_{\zeta-1,t}^{w^*_t}\}\cdot \big|(w_t^*)^\top(\hat\theta_{\zeta-1,t}-\theta)\big|.
\label{eq:xjstar-expansion-2}
\end{align}
In addition, because both $y^*_t$ and $w^*_t$ belong to $\mathcal N_{\zeta,t} \subseteq \mathcal N_{\zeta - 1,t}$, the second step of Algorithm \ref{alg:suplinucb} implies that 
\begin{equation}
(y_t^*)^\top\hat\theta_{\zeta-1,t} \leq (w_t^*)^\top\hat\theta_{\zeta-1,t} - 2^{1-(\zeta-1)} \leq (w_t^*)^\top\hat\theta_{\zeta-1,t}-2^{2-\zeta},
\label{eq:xijstar-side-2}
\end{equation}
and
\begin{equation}
 \varpi_{\zeta-1,t}^{y^*_t} \leq 2^{-(\zeta -1)}, \qquad  \varpi_{\zeta-1,t}^{w^*_t} \leq 2^{-(\zeta -1)} .
\label{eq:xijstar-side-3}
\end{equation}
Subtracting Eq.~(\ref{eq:xistar-expansion-2}) from Eq.~(\ref{eq:xjstar-expansion-2}) and applying Eqs.~(\ref{eq:xijstar-side-2},\ref{eq:xijstar-side-3}), we get
\begin{align*}
 \overline m_{\zeta,t}& -\underline m_{\zeta,t}  = (y_t^*-w_t^*) \\
& \leq 2^{2-\zeta} +  2 \cdot 2^{-(\zeta -1)}  +  \vct 1\{\neg\mathcal E_{\zeta-1,t}^{y^*_t}\}\cdot \big|(y_t^*)^\top(\hat\theta_{\zeta-1,t}-\theta)\big| +  1\{\neg\mathcal E_{\zeta-1,t}^{w^*_t}\}\cdot \big|(w_t^*)^\top(\hat\theta_{\zeta-1,t}-\theta)\big| \\
& = 2^{3-\zeta}  +  \vct 1\{\neg\mathcal E_{\zeta-1,t}^{y^*_t}\}\cdot \big|(y_t^*)^\top(\hat\theta_{\zeta-1,t}-\theta)\big| +  1\{\neg\mathcal E_{\zeta-1,t}^{w^*_t}\}\cdot \big|(w_t^*)^\top(\hat\theta_{\zeta-1,t}-\theta)\big| .
\end{align*}
Therefore, we have
\[
\E\left[\max\{ \overline m_{\zeta,t} -\underline m_{\zeta,t}  - 2^{3-\zeta}, 0\}\right] \leq \vct 1\{\neg\mathcal E_{\zeta-1,t}^{y^*_t}\}\cdot \big|(y_t^*)^\top(\hat\theta_{\zeta-1,t}-\theta)\big| +  1\{\neg\mathcal E_{\zeta-1,t}^{w^*_t}\}\cdot \big|(w_t^*)^\top(\hat\theta_{\zeta-1,t}-\theta)\big| .
\]
We finally apply Lemma \ref{lem:reward-error-bound-in-each-layer} and prove Eq.~(\ref{eq:mt-2}).
\end{proof}



% Let $x_{i^*, t} \in D_t$ be a candidate arm that maximizes the mean reward $\langle x_{i^*, t},  \theta\rangle$ at time $t$. It is straightforward to verify that the same proof for Lemma~\ref{lem:reward-error-bound-in-each-layer} yields the following statement.
% \begin{lemma}\label{lem:best-arm-reward-error-bound-in-each-layer}
% There exists a universal constant $\xi > 0$ such that for each layer $\zeta$ 
% and for each time $t \in \cN_\zeta$, 
% it holds that
% \begin{align*}
% \E\left[\left| (x_{i^*, t})^\top (\hat{\theta}_{\zeta, t} - \theta)\right|\right] < \xi \left( \E \left[(\sqrt{d} + \alpha_{\zeta, t}^{i^*}) \omega_{\zeta, t}^{i^*}\right] + d \sqrt{\log T / T} \right).
% \end{align*}
% \end{lemma}

% Combining Lemma~\ref{lem:reward-error-bound-in-each-layer} and Lemma~\ref{lem:best-arm-reward-error-bound-in-each-layer}, we are able to prove Lemma~\ref{lem:single-step-regret}, as follows.
% \begin{proof}[Proof of Lemma~\ref{lem:single-step-regret}] Note that
% \begin{align}
% &\E\left[ \sup_{i \in [n]}\langle x_{it}, \theta\rangle -  \langle x_{i_t, t}, \theta\rangle \right]  = \E\left[\langle x_{i^*, t}, \theta\rangle  - \langle x_{i_t, t}, \theta\rangle   \right] \nonumber \\
% &\qquad\qquad \leq  \E\left[\langle x_{i^*, t}, \hat{\theta}_{\zeta, t}\rangle  + \left|\langle x_{i^*, t}, \hat{\theta}_{\zeta, t} - \theta\rangle\right|  - \langle x_{i_t, t}, \theta\rangle   \right]  \nonumber \\
% &\qquad \qquad \leq  O\left(d \sqrt{\log T/T}\right) +  \E\left[\langle x_{i^*, t}, \hat{\theta}_{\zeta, t}\rangle  + C (\sqrt{d} + \alpha_{\zeta, t}^{i^*}) \omega_{\zeta, t}^{i^*}   - \langle x_{i_t, t}, \theta\rangle   \right] , \label{eq:cor-single-step-regret-1}
% \end{align}
% where the last inequality is because of Lemma~\ref{lem:best-arm-reward-error-bound-in-each-layer}, so long as $C \geq \xi$. 
% By Line~\ref{line:alg-4} of Algorithm~\ref{alg:suplinucb}, we have that 
% $\langle x_{i^*, t}, \hat{\theta}_{\zeta, t}\rangle  + C (\sqrt{d} + \alpha_{\zeta, t}^{i^*}) \omega_{\zeta, t}^{i^*} \leq \langle x_{i_t, t}, \hat{\theta}_{\zeta, t}\rangle  + C (\sqrt{d} + \alpha_{\zeta, t}^{i_t}) \omega_{\zeta, t}^{i_t}$, 
% and therefore, continuing with Eq.~\ref{eq:cor-single-step-regret-1}, we have
% \begin{align*}
% \E\left[ \sup_{i \in [n]}\langle x_{it}, \theta\rangle -  \langle x_{i_t, t}, \theta\rangle \right] &\leq  O\left(d \sqrt{\log T/T}\right) +  \E\left[C (\sqrt{d} + \alpha_{\zeta, t}^{i_t}) \omega_{\zeta, t}^{i_t} + \langle x_{i_t, t}, \hat{\theta}_{\zeta, t}\rangle    - \langle x_{i_t, t}, \theta\rangle   \right] \\
% & \lesssim d\sqrt{\log T / T} + \E\left[ (\sqrt{d} + \alpha_{\zeta, t}^{i_t}) \omega_{\zeta, t}^{i_t}\right] ,
% \end{align*}
% where the last inequality is because of Lemma~\ref{lem:reward-error-bound-in-each-layer}.
% \end{proof}
